Fuel Efficient Computation in Passive Self-Assembly

In this paper we show that passive self-assembly in the context of the tile self-assembly model is capable of performing fuel efficient, universal computation. The tile self-assembly model is a premiere model of self-assembly in which particles are modeled by four-sided squares with glue types assigned to each tile edge. The assembly process is driven by positive and negative force interactions between glue types, allowing for tile assemblies floating in the plane to combine and break apart over time. We refer to this type of assembly model as passive in that the constituent parts remain unchanged throughout the assembly process regardless of their interactions. A computationally universal system is said to be fuel efficient if the number of tiles used up per computation step is bounded by a constant. Work within this model has shown how fuel guzzling tile systems can perform universal computation with only positive strength glue interactions. Recent work has introduced space-efficient, fuel-guzzling universal computation with the addition of negative glue interactions and the use of a powerful non-diagonal class of glue interactions. Other recent work has shown how to achieve fuel efficient computation within active tile self-assembly. In this paper we utilize negative interactions in the tile self-assembly model to achieve the first computationally universal passive tile self-assembly system that is both space and fuel-efficient. In addition, we achieve this result using a limited diagonal class of glue interactions.

==> definitions.tex <==

\section{Definitions and Model}

\subsection{Tile Self-Assembly Model}
\paragraph{Tiles.}  Consider some alphabet of glue types $\Pi$.  A tile is a finite edge polygon with some finite subset of border points each assigned some glue type from $\Pi$.  Further, each glue type $g \in \Pi$ has some integer strength $str(g)$.  In this paper we consider a special class of tiles that are unit squares of the same orientation with at most one glue type per face, with each glue being placed exactly in the center of the tile's face.

\paragraph{Assemblies.}  An assembly is a set of tiles whose interiors do not overlap.  For a given assembly $\Upsilon$, define the \emph{bond} graph $G_\Upsilon$ to be the weigthed graph in which each element of $\Upsilon$ is a vertex, and each edge weight between tiles is the sum of the strengths of the overlapping, matching glue points of the two tiles.  For an assembly $C$ and a cut of $G_C$ into assemblies $A$ and $B$ with weight $r$, we say that $C$ is $\tau$-breakable into $A$ and $B$ for any $\tau > r$.  For an assembly $C$ with min-cut at least $\tau$, we say that $C$ is $\tau$-stable.  Note that any assembly in which the set of border points of all tiles in the assembly is not a connected set will not be $\tau$-stable for any $\tau > 0$.


\paragraph{Transitions.}  Two assemblies can potentially combine into a third, new assembly, or a single assembly can potentially break into two smaller assemblies.  Each type of transition is defined in terms of the temperature threshold $\tau$ of the system.
    \begin{itemize}
        \item    - combination.  Consider two assemblies $A$ and $B$.  If $B$ can be translated into $B'$ such that $A \bigcup B'$ is a valid (not overlapping), $\tau$-stable assembly, then we say that $A$ and $B$ may combine into $C$ at temperature $\tau$.
        \item - separation.  Consider an assembly $C$ that is not $\tau$-stable.  Then, for any $A$ and $B$ such that $C$ is $\tau$-breakable into $A$ and $B$ we say that $C$ may separate into $A$ and $B$ at temperature $\tau$.
    \end{itemize}

\paragraph{Tile Assembly System $(T,\tau)$.}  A (2-handed) tile assembly system is an ordered pair $(T,\tau)$ where $T$ is a set of initial assemblies, and $\tau$ is a positive integer referred to as the \emph{temperature} of the system.  A tile system has an associated set of \emph{producible} assemblies, \emph{$PROD_{T,\tau}$}, which define what can be built by the system.  Formally, $T \subseteq PROD_{T,\tau}$ as a base case set of assemblies.  Further, given any $A,B \in PROD_{T,\tau}$ with $A$ and $B$ $\tau$-combinable into $C$, then $C \in PROD_{T,\tau}$, and for any $C \in PROD_{T,\tau}$ where $C$ is $\tau$-breakable into $A$ and $B$, then $A,B \in PROD_{T,\tau}$.  Put another way, the set of producible assemblies contains any assembly that can be obtained by a valid sequence of combinations and breaks, starting from the initial set of assemblies $T$.

\subsection{Misc. Definitions.}

\paragraph{Directed Graph.}  A directed graph $G = (V, E)$ is a duple where $V$ is the set of vertices and $E$ is a set of ordered pairs of vertices. For all $e \in E$, $e = (x, y)$ is a directed connection from $x \to y$. A valid walk $w$ of $G$ is a sequence of vertices $<w_0, w_1, w_2, ... , w_i, ..., w_k>$ such that either $w = \emptyset$ or $\forall w_i \in w \exists e \in E(e = (w_{i^{th}}, w_{(i+1)^{th}}))$ when $w_i$ is not equal to $w_k$.

\paragraph{Valid Assembly Sequence.}  Given a tile set $T$ an assembly sequence $AS$ is a sequence of assemblies taken from the tile set $T$. A valid assembly sequence of the tile set $T$ must only contain assemblies from $PROD_T$ and the $(i+1)^{th}$ assembly in the sequence must either be a valid combination of the $i^{th}$ assembly with another assembly in $PROD_T$ or a valid break of the $i^{th}$ assembly. Then, the set of all valid assembly sequences in a tile set $T$ is $T_{AS}$.

\subsection{Problem Formulation:  Oscillators, etc..}
A system is an oscillator if... We want some special assembly to be marked as 'red' or something.  Over time, this marked assembly can grow, or break down.  We are always interested in the piece that is marked (in the case it breaks, we are interested in the piece that contains the marked portion of the assembly).  Then, to be an oscillator, all assembly sequences that deal with the marked assembly must switch back and forth between a '0' assembly and a '1' assembly infinitely often, and the number of transition assemblies between each 0,1 transition must be bounded by some constant.  By this definition, we will have the first tile self-assembly oscillator result.  This concept needs to be formalized.

